Detecting Anomalies within Smart Buildings using Do-It-Yourself Internet of Things

Detecting anomalies at the time of happening is vital in environments like buildings and homes to identify potential cyber-attacks. This paper discussed the various mechanisms to detect anomalies as soon as they occur. We shed light on crucial considerations when building machine learning models. We constructed and gathered data from multiple self-build (DIY) IoT devices with different in-situ sensors and found effective ways to find the point, contextual and combine anomalies. We also discussed several challenges and potential solutions when dealing with sensing devices that produce data at different sampling rates and how we need to pre-process them in machine learning models. This paper also looks at the pros and cons of extracting sub-datasets based on environmental conditions.

==> Reviewers_Comments.tex <==
COMMENTS TO THE AUTHOR:

Reviewer #1:
1) The authors have  used various anomaly detection techniques to detect anomalous behaviour within a building using IoT sensors. The paper is readable but needs improvements. The paper provides a lot of practical insights towards anomaly detection using DIY IoT devices.  Lost of casual language has been used that required revising.
ACTION
Review the language

2) The paper mentioned a link that does not work.
ACTION
Supply link to github/gitlab

3) There are types that need to be corrected e.g. Co2 need subscript, Figure needs to be capitalised, Equation needs to be capitalised.
Action: Correct types and capitalise equations

4) Section 4.2 seems to be quite small and need to be better integrated with the rest of the section
Action: Make section 4.2 better
Status: Done

5) Captions need to be meaningful. E.g. Figure 13-14 captions are not self-contained. Explain the mars within each figure.
ACTION
Correct figure captions

6) Lessons leant section need to be better structured. It is difficult to follow. It would be useful to make each lesson explained separately.
ACTION
Structure lessons learnt section

6) X and y axis of both figures are not readable. Font size needs to be increased.
ACTION
Increase font sizes


Reviewer #2: This article approaches the problem of detecting anomalies in IoT based buildings. The proposed solution uses relevant methods from machine learning. The addressed problem is of important scientific and practical relevance and the scientific contributions are good.

However, the paper should fix the following important issues:
1)- The notion of anomaly is central and should be defined and exemplified. Are you also dealing with the security anomalies? If not, does the proposed solution can be extended further to take them into account.


2)- the data that is used in validating the different methods should be discussed. How were they collected and managed? How representative are they for various types of anomalies?
3)- The originality of the solution relative to existing works should be further discussed by focusing on the exploited methods, the efficiency and the cost of each solution.
4)- The obtained results should be further discussed to showcase the efficacy of the solution as well as its cost.
5)- The paper findings should be also summarized in the conclusion.


Reviewer #3: The paper focuses on detecting anomalies using sensors within buildings. This is a fairly well-written piece of work. They have used well-known anomaly detection techniques and used them to detect anomalies. The authors have discussed a series of steps they have dace to process the pre-collected data stream. The paper provides valuable insights toward developing a real-world anomaly detection pipeline for tackling building data. However, the following issues need to be addressed.

(1) It is not clear what the authors mean by "pros and cons of extracting sub-datasets". Please clarify
(2) The link is not provided as mentioned at the end of section 1
(3) Device setup is not clear. Try to use a figure explicitly showing the sensors and data streams and the overall data architecture.
(4) Paper refer to table 2.4 but the actual caption is missing. Please clarify. Further, this table is difficult to read. Authors are encouraged to use some type of colour-coding to improve the readability
(5) Figures need to be better labelled. Authors are encouraged to use subfigures to avoid Figures numbers getting increased unnecessarily. Captions need to be improved by adding left and right labels on the caption itself
(6) It is not clear how the threshold being selected around Equation 9 and 10
(7) Not all symbols are explained in E.q 9
(8) Section 4.2 seems too small to either remove or expand. Perhaps it would be good to incorporate a table that compares different types of anomaly detection work carried out within buildings and the types of sensors they have used.
(8) Paper need to be proofread to improve its readability. Some sections are difficult to read
(9) There are some inconsistencies in the use of abbreviations e.g. SKLearn and SKL

